Efficient Wasserstein Natural Gradients for Reinforcement Learning

A novel optimization approach is proposed for application to policy gradient methods and evolution strategies for reinforcement learning (RL). The procedure uses a computationally efficient Wasserstein natural gradient (WNG) descent that takes advantage of the geometry induced by a Wasserstein penalty to speed optimization. This method follows the recent theme in RL of including a divergence penalty in the objective to establish a trust region. Experiments on challenging tasks demonstrate improvements in both computational cost and performance over advanced baselines.

==> kwng_rl (1)/m.macros.tex <==
\makeatletter

\newcommand{\define}[1]{{\bf #1}}
\newcommand{\figpanel}[1]{\textsf{#1}}
\newcommand{\todo}[1]{}
%\newcommand{\todo}[1]{[\textit{TODO: #1}]}

% some abbreviations

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}

\newcommand{\intinf}{\int_{-\infty}^{+\infty}}

% reference styles
\newcommand{\chpref}[1]{chapter~\ref{chp:#1}}
\newcommand{\Chpref}[1]{Chapter~\ref{chp:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[2]{figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\Figref}[2]{Figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\eqnref}[1]{(\ref{eqn:#1})}
\newcommand{\Eqnref}[1]{Equation (\ref{eqn:#1})}

% set horizontal margins to center text (using current paperwidth & textwidth)
\def\equalmargins{
	\setlength{\oddsidemargin}{\paperwidth}
	\addtolength{\oddsidemargin}{-\textwidth}
	\setlength{\oddsidemargin}{0.5 \oddsidemargin}
	\addtolength{\oddsidemargin}{-1in}
	\setlength{\evensidemargin}{\oddsidemargin}
}


% force equation numbers
\newenvironment{eqnforce}[1]{%
\let\savetheequation=\theequation% save the old equation number defn
\renewcommand{\theequation}{#1}%   set the equation string
\begin{equation}%		   start a normal equation env
}{%
\end{equation}%			   end it
\let\theequation=\savetheequation% restore the old defn
\addtocounter{equation}{-1}%       restore the counter which was incremented
}

% abbreviate \nonumber\\
\newcommand{\nn}{\nonumber\\}

% make text in super/subscripts the right size
\newcommand\mathbox[1]{\mathchoice{\mbox{#1}}{\mbox{#1}}%
{\mbox{\scriptsize{#1}}}{\mbox{\tiny{#1}}}}


% et al.
\newcommand{\etal}{\textit{et al$.$}}

% move the control point of the argument to the bottom of the box ...
\def\alignbottom#1{%
  \setbox0=\hbox{#1}%
  \raise\dp0\box0%
}
% ... or to the top ...
\newcommand{\aligntop}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=-\ht0%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}
% ... or to the middle.

\newcommand{\alignmiddle}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=\dp0%
  \advance\dimen0 by -\ht0%
  \divide\dimen0 by 2%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ tricks

\RequirePackage{tikz}

%% Create inline node: shorthand for \tikz[baseline,OPT1]{\node [OPT2] {ARG}}
%% some uses:
%% \tikznode[base]{foo}   
%% \tikznode[middle]{foo} 
%% \tikznode[below]{foo}
%% \tikznode[below=-1ex]{foo}
%% \tikznode[draw=red]{foo}       % tight red frame
%% \tikznode[framed=blue]{foo}    % adds some space (can be adjusted w/ inner sep
\newcommand\tikznode[1][]{%
  \@ifnextchar[{\m@tikznode[#1]}{\m@tikznode[][#1]}}
\def\m@tikznode[#1][#2]#3{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
  \tikz[baseline,#1]{\node [anchor=base,inner sep=0pt, #2] {#3};}%
  \endgroup%
}

%% Option to \path to annotate within a node (eg place text on a figure):
%% \node (fig) {\includegraphics{}};
%% \path[fit to node=fig] (0.1, 1) node {A};
\tikzoption{fit to node}{\tikzset{shift=(#1.south west), x=(#1.south east), y=(#1.north west)}}


%% Create inline node with pin label box pointing to content
%% \tikznodepin[env opts][inline node opts]{inline text}(pos)[pinnode
%% opts][pin edge opts]{pin text}

\tikzstyle{tikznode label node}=[]
\tikzstyle{tikznode label edge}=[->, very thick]
\tikzoption{tikznode label position}{#1\tikznodelabel@setposition#1}
\def\tikznodelabel@setposition(#1){\def\tikznodelabel@position{#1}}
\def\tikznodelabel@position{0, 5ex}

\def\tikznodelabel{%
  \@ifnextchar[{\tikznodelabel@m}{\tikznodelabel@@m[][]}
}
\def\tikznodelabel@m[#1]{%
  \@ifnextchar[{\tikznodelabel@@m[#1]}{\tikznodelabel@@m[][#1]}
}
\def\tikznodelabel@@m[#1][#2]#3{%
  \@ifnextchar({\tikznodelabel@@@m[#1][#2]{#3}}
               {\tikznodelabel@@@m[#1][#2]{#3}(\tikznodelabel@position)}
}
\def\tikznodelabel@@@m[#1][#2]#3(#4){%
  \@ifnextchar[{\tikznodelabel@@@@m[#1][#2]{#3}(#4)}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[][]}
}
\def\tikznodelabel@@@@m[#1][#2]#3(#4)[#5]{%
  \@ifnextchar[{\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5]}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5][]}
}
\def\tikznodelabel@@@@@m[#1][#2]#3(#4)[#5][#6]#7{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
%
  \tikz[baseline,#1]{
    \node (inl) [anchor=base,inner sep=0pt, #2] {#3};
    \useasboundingbox;
    \path (#4) node [tikznode label node, #5] {#7} 
               edge [tikznode label edge, #6] (inl);
   }%
  \endgroup%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parse a comma-separated list.  
%
% Latex provides \@for\var=first,second,...,last\do{code} which
% executes {code} many times, each time setting \var to the next item in
% the list 
% 
% This provides a variant \@forlast\var:=a,b,...,z\do{code}{codelast}
% which differs only on the last entry, for which it executes {codelast}.

\long\def\@forlast#1:=#2\do#3#4{%
  \expandafter\def\expandafter\@forlasttmp\expandafter{#2}%
  \ifx\@forlasttmp\@empty%
  \else%
    \expandafter\@forlastloop#2,\@nil,\@nil\@@#1{#3}{#4}%
  \fi%
}

\long\def\@forlastloop#1,#2,#3\@@#4#5#6{%
  \def#4{#1}%
  \ifx #4\@nnil%
    % empty list -- do nothing
  \else%
    \ifx #2\@nil% check if single item
      #6% apply #6 to #1
    \else%
      #5% apply #5 to #1
      \@forlastloop#2,#3\@@#4{#5}{#6}
    \fi%
  \fi%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Grab this page from an image file.  Can be used for a background.
%%   This version works 

%\newcommand\pageimage[1]{%
%  \hspace{-\oddsidemargin}\hspace*{-1in}%
%  \vspace*{-\topmargin}\vspace*{-\headheight}\vspace*{-\headsep}\vspace*{-1in}%
%  \makebox[top,left](0,0)\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio}{#1}
%} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% panel sizes.  

\let\panelwidth\columnwidth
\let\panelheight\textheight


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% image resizing.  width and height give maxima in terms of
%%   columnwidth and textheight respectively.

\def\parsesize[#1,#2]{{#1\panelwidth}{#2\panelheight}}

%% column image is deprecates

\def\mycolumnimage[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}
\newcommand{\columnimage}[2][1,.98]{\mycolumnimage[#1][]{#2}}

\def\mycenterimage[#1,#2][#3]#4{%
  \begin{center}\mycolumnimage[#1,#2][#3]{#4}\end{center}}



\newcommand{\centerimage}[2][1,.98]{\mycenterimage[#1][]{#2}}

\def\myvcenterimage[#1,#2][#3]#4{%
  \vfill\mycenterimage[#1,#2][#3]{#4}\vfill}
\newcommand{\vcenterimage}[2][1,.98]{\myvcenterimage[#1][]{#2}}

\newcommand{\columnline}[2][1]{\hbox to #1\panelwidth{#2}}
\renewcommand{\centerline}[2][1]{\hbox to #1\panelwidth{\hfil #2 \hfil}}


\newcommand{\columnimagestack}[2][1,.98]{%
  \@forlast\n@xtimg:=#2\do%
     {\makebox(0,0)[lb]{\mycolumnimage[#1][]{\n@xtimg}}}%
     {\mycolumnimage[#1][]{\n@xtimg}}%
}

%% so is scaleimage

\def\ScaleImgTwoOpt[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}

\def\ScaleImgOneOpt[#1,#2]{%
  \@ifnextchar[%]
    {\ScaleImgTwoOpt[#1,#2]}%
    {\ScaleImgTwoOpt[#1,#2][]}%
}

\def\scaleimage{%
  \@ifnextchar[%]
    {\ScaleImgOneOpt}%
    {\ScaleImgOneOpt[1,1]}%
}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% beamer extensions
\@ifclassloaded{beamer}{

%% Beamer controlled underbrace.  
%% \underbraceon<spec>[prefix]{maintext}{subtext}
%%   - prefix should probably live outside the \alt anyway
\newcommand<>{\underbraceon}[3][]{%
  \alt#4{%
    {#1{\underset{#3}{\underset{\text{\upbracefill}}{#2}}}}
  }{
    {#1{\underset{\phantom{#3}}{\underset{\phantom{\text{\upbracefill}}}{#2}}}}
  }%
}

} % end if beamer



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pgf extensions

\def\pgfp@nelparsearg[#1,#2]{%
  \def\pgfp@nelwidth{#1\panelwidth}%
  \def\pgfp@nelheight{#2\panelheight}}

\newenvironment{pgfpanel}[1][1,.995]
  {\pgfp@nelparsearg[#1]
   \begin{pgfpicture}{0cm}{0cm}{\pgfp@nelwidth}{\pgfp@nelheight}
      \pgftranslateto{\pgfpoint{0cm}{\pgfp@nelheight}}
      \pgfsetxvec{\pgfpoint{\pgfp@nelwidth}{0cm}}
      \pgfsetyvec{\pgfpoint{0cm}{-\pgfp@nelheight}}}
  {\end{pgfpicture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these use pgf to place a box at an arbitrary spot and (second form)
%% draw an arrow to the current position

\newcommand\placebox[4][left,baseline]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfputat{\pgfpoint{#2}{#3}}{\pgfbox[#1]{#4}}
  \end{pgfpicture}%
}

\newcommand\arrowbox[4][{0cm}{0cm}]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfnodebox{text}[virtual]{\pgfpoint{#2}{#3}}{#4}{2pt}{2pt}
    \pgfnodecircle{origin}[virtual]{\pgfpoint#1}{0pt}
    \pgfsetlinewidth{.5mm}
    \pgfsetendarrow{\pgfarrowsingle}
    \pgfnodeconnline{text}{origin}
  \end{pgfpicture}
}




% \def\alignmiddle#1{%
%   \setbox0=\hbox{#1}%
%   \dimen0=\dp0%
%   \advance\dimen0 by -\ht0%
%   \divide\dimen0 by 2%
%   \raise\dimen0\box0%
% }


\makeatother


==> kwng_rl (1)/m.symbols.tex <==
\RequirePackage{ifthen}

% use | for math mode
%\catcode`\|=3

% use textmode for a short minus sign
\newcommand{\tminus}{\text{\textendash}}

% vector
\newcommand{\vx}{\vec x}

% symbols for probability distributions
\newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
\newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
\newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}
% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\lr]{x} -> \mathbb{E}_a \lr[ x \lr]
\makeatletter
\def\expect{\@ifnextchar[{\expect@}{\expect@@[][\lr]}}
\def\expect@[#1]{\@ifnextchar[{\expect@@[#1]}{\expect@@[#1][\lr]}}
\def\expect@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{E}\newlr#2[{#3}#2]}%
             {\mathbb{E}_{#1}\newlr#2[{#3}#2]}}
\def\var{\@ifnextchar[{\var@}{\var@@[][\lr]}}
\def\var@[#1]{\@ifnextchar[{\var@@[#1]}{\var@@[#1][\lr]}}
\def\var@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{V}\newlr#2[{#3}#2]}%
             {\mathbb{V}_{#1}\newlr#2[{#3}#2]}}
\makeatother
\newcommand{\angles}[2][\lr]{{\newlr #1\langle{#2}#1\rangle}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathcal{E}}{=}}
% likelihoods
\newcommand{\like}[2]{\ensuremath{{\cal L}_{#1}\left({#2}\right)}}
\newcommand{\loglike}[2]{\ensuremath{\ell_{#1}\left({#2}\right)}}
\newcommand{\eff}{\mathcal{F}}
% info theoretic
\newcommand{\entropy}[2][\lr]{\ensuremath{\textbf{\textsf{H}}%
                             {\newlr #1[{#2}#1]}}}
\def\mutualinfo[#1;#2]{\ensuremath{\textbf{\textsf{I}}[{#1};{#2}]}}
\newcommand{\KL}[3][\lr]{\ensuremath{\textbf{\textsf{KL}}%
                             {\newlr #1[{#2}\lrmid #1\|{#3}#1]}}}
\newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
\newcommand{\normal}[3][\lr]{\ensuremath{\newlr\mathcal{N}#1(#2,#3#1)}}

% fractions
\newcommand{\half}{\ensuremath{{1\over2}}}
\newcommand{\overN}{\ensuremath{{1\over N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}

% whitened quantities
\newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\setV}{\ensuremath{{\cal V}}}
\newcommand{\setX}{\ensuremath{{\cal X}}}
\newcommand{\setY}{\ensuremath{{\cal Y}}}
\newcommand{\setZ}{\ensuremath{{\cal Z}}}
\newcommand{\size}[1]{\ensuremath{\left\vert{#1}\right\vert}}

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
\renewcommand{\vec}[1]{\ensuremath{\mathchoice%
{\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
{\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
\newcommand{\norm}[2][\lr]{\ensuremath{\newlr#1\|#2#1\|}}
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\renewcommand{\det}[2][\lr]{\ensuremath{\newlr#1\vert{#2}#1\vert}}
\newcommand{\trace}[2][\lr]{\ensuremath{\newlr\mathsf{Tr}#1[{#2}#1]}}
\newcommand{\diag}[2][\lr]{\ensuremath{\newlr\mathbox{\textsf{diag}}#1[{#2}#1]}}


% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\newcommand{\intdx}[1][dx]{\int\!\!#1\,}

\newcounter{multintctr}
\newcommand{\mltint}[1][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \int}

\newcommand{\mltintdx}[2][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \intdx[#2]}

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}


% accents

% adapted from symbols-a4.pdf; optional args permit shortening at left
% and right ends
\makeatletter
\def\widebar{\@ifnextchar[{\widebar@}{\widebar@@[3][0]}}
\def\widebar@[#1]{\@ifnextchar[{\widebar@@[#1]}{\widebar@@[#1][0]}}
\def\widebar@@[#1][#2]#3{{}\mkern#1mu\mkern#2mu\overline{\mkern-#1mu#3\mkern-#2mu}}
\makeatother    
        

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}


\newboolean{inlr}
\newboolean{midlr}
\setboolean{inlr}{false}
\newcommand\newlr{\setboolean{inlr}{false}}

\newcommand\lr[1]{%
  \ifthenelse{\boolean{inlr}}%
    {\ifthenelse{\boolean{midlr}}%
      {\middle#1\setboolean{inlr}{true}}
      {\right#1}}%
    {\left#1\setboolean{inlr}{true}}}%
\newcommand\lrmid{%
  \ifthenelse{\boolean{inlr}}%
    {\setboolean{midlr}{true}}
    {}}%



==> kwng_rl (1)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> m.macros.tex <==
\makeatletter

\newcommand{\define}[1]{{\bf #1}}
\newcommand{\figpanel}[1]{\textsf{#1}}
\newcommand{\todo}[1]{}
%\newcommand{\todo}[1]{[\textit{TODO: #1}]}

% some abbreviations

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}

\newcommand{\intinf}{\int_{-\infty}^{+\infty}}

% reference styles
\newcommand{\chpref}[1]{chapter~\ref{chp:#1}}
\newcommand{\Chpref}[1]{Chapter~\ref{chp:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[2]{figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\Figref}[2]{Figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\eqnref}[1]{(\ref{eqn:#1})}
\newcommand{\Eqnref}[1]{Equation (\ref{eqn:#1})}

% set horizontal margins to center text (using current paperwidth & textwidth)
\def\equalmargins{
	\setlength{\oddsidemargin}{\paperwidth}
	\addtolength{\oddsidemargin}{-\textwidth}
	\setlength{\oddsidemargin}{0.5 \oddsidemargin}
	\addtolength{\oddsidemargin}{-1in}
	\setlength{\evensidemargin}{\oddsidemargin}
}


% force equation numbers
\newenvironment{eqnforce}[1]{%
\let\savetheequation=\theequation% save the old equation number defn
\renewcommand{\theequation}{#1}%   set the equation string
\begin{equation}%		   start a normal equation env
}{%
\end{equation}%			   end it
\let\theequation=\savetheequation% restore the old defn
\addtocounter{equation}{-1}%       restore the counter which was incremented
}

% abbreviate \nonumber\\
\newcommand{\nn}{\nonumber\\}

% make text in super/subscripts the right size
\newcommand\mathbox[1]{\mathchoice{\mbox{#1}}{\mbox{#1}}%
{\mbox{\scriptsize{#1}}}{\mbox{\tiny{#1}}}}


% et al.
\newcommand{\etal}{\textit{et al$.$}}

% move the control point of the argument to the bottom of the box ...
\def\alignbottom#1{%
  \setbox0=\hbox{#1}%
  \raise\dp0\box0%
}
% ... or to the top ...
\newcommand{\aligntop}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=-\ht0%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}
% ... or to the middle.

\newcommand{\alignmiddle}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=\dp0%
  \advance\dimen0 by -\ht0%
  \divide\dimen0 by 2%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ tricks

\RequirePackage{tikz}

%% Create inline node: shorthand for \tikz[baseline,OPT1]{\node [OPT2] {ARG}}
%% some uses:
%% \tikznode[base]{foo}   
%% \tikznode[middle]{foo} 
%% \tikznode[below]{foo}
%% \tikznode[below=-1ex]{foo}
%% \tikznode[draw=red]{foo}       % tight red frame
%% \tikznode[framed=blue]{foo}    % adds some space (can be adjusted w/ inner sep
\newcommand\tikznode[1][]{%
  \@ifnextchar[{\m@tikznode[#1]}{\m@tikznode[][#1]}}
\def\m@tikznode[#1][#2]#3{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
  \tikz[baseline,#1]{\node [anchor=base,inner sep=0pt, #2] {#3};}%
  \endgroup%
}

%% Option to \path to annotate within a node (eg place text on a figure):
%% \node (fig) {\includegraphics{}};
%% \path[fit to node=fig] (0.1, 1) node {A};
\tikzoption{fit to node}{\tikzset{shift=(#1.south west), x=(#1.south east), y=(#1.north west)}}


%% Create inline node with pin label box pointing to content
%% \tikznodepin[env opts][inline node opts]{inline text}(pos)[pinnode
%% opts][pin edge opts]{pin text}

\tikzstyle{tikznode label node}=[]
\tikzstyle{tikznode label edge}=[->, very thick]
\tikzoption{tikznode label position}{#1\tikznodelabel@setposition#1}
\def\tikznodelabel@setposition(#1){\def\tikznodelabel@position{#1}}
\def\tikznodelabel@position{0, 5ex}

\def\tikznodelabel{%
  \@ifnextchar[{\tikznodelabel@m}{\tikznodelabel@@m[][]}
}
\def\tikznodelabel@m[#1]{%
  \@ifnextchar[{\tikznodelabel@@m[#1]}{\tikznodelabel@@m[][#1]}
}
\def\tikznodelabel@@m[#1][#2]#3{%
  \@ifnextchar({\tikznodelabel@@@m[#1][#2]{#3}}
               {\tikznodelabel@@@m[#1][#2]{#3}(\tikznodelabel@position)}
}
\def\tikznodelabel@@@m[#1][#2]#3(#4){%
  \@ifnextchar[{\tikznodelabel@@@@m[#1][#2]{#3}(#4)}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[][]}
}
\def\tikznodelabel@@@@m[#1][#2]#3(#4)[#5]{%
  \@ifnextchar[{\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5]}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5][]}
}
\def\tikznodelabel@@@@@m[#1][#2]#3(#4)[#5][#6]#7{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
%
  \tikz[baseline,#1]{
    \node (inl) [anchor=base,inner sep=0pt, #2] {#3};
    \useasboundingbox;
    \path (#4) node [tikznode label node, #5] {#7} 
               edge [tikznode label edge, #6] (inl);
   }%
  \endgroup%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parse a comma-separated list.  
%
% Latex provides \@for\var=first,second,...,last\do{code} which
% executes {code} many times, each time setting \var to the next item in
% the list 
% 
% This provides a variant \@forlast\var:=a,b,...,z\do{code}{codelast}
% which differs only on the last entry, for which it executes {codelast}.

\long\def\@forlast#1:=#2\do#3#4{%
  \expandafter\def\expandafter\@forlasttmp\expandafter{#2}%
  \ifx\@forlasttmp\@empty%
  \else%
    \expandafter\@forlastloop#2,\@nil,\@nil\@@#1{#3}{#4}%
  \fi%
}

\long\def\@forlastloop#1,#2,#3\@@#4#5#6{%
  \def#4{#1}%
  \ifx #4\@nnil%
    % empty list -- do nothing
  \else%
    \ifx #2\@nil% check if single item
      #6% apply #6 to #1
    \else%
      #5% apply #5 to #1
      \@forlastloop#2,#3\@@#4{#5}{#6}
    \fi%
  \fi%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Grab this page from an image file.  Can be used for a background.
%%   This version works 

%\newcommand\pageimage[1]{%
%  \hspace{-\oddsidemargin}\hspace*{-1in}%
%  \vspace*{-\topmargin}\vspace*{-\headheight}\vspace*{-\headsep}\vspace*{-1in}%
%  \makebox[top,left](0,0)\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio}{#1}
%} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% panel sizes.  

\let\panelwidth\columnwidth
\let\panelheight\textheight


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% image resizing.  width and height give maxima in terms of
%%   columnwidth and textheight respectively.

\def\parsesize[#1,#2]{{#1\panelwidth}{#2\panelheight}}

%% column image is deprecates

\def\mycolumnimage[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}
\newcommand{\columnimage}[2][1,.98]{\mycolumnimage[#1][]{#2}}

\def\mycenterimage[#1,#2][#3]#4{%
  \begin{center}\mycolumnimage[#1,#2][#3]{#4}\end{center}}



\newcommand{\centerimage}[2][1,.98]{\mycenterimage[#1][]{#2}}

\def\myvcenterimage[#1,#2][#3]#4{%
  \vfill\mycenterimage[#1,#2][#3]{#4}\vfill}
\newcommand{\vcenterimage}[2][1,.98]{\myvcenterimage[#1][]{#2}}

\newcommand{\columnline}[2][1]{\hbox to #1\panelwidth{#2}}
\renewcommand{\centerline}[2][1]{\hbox to #1\panelwidth{\hfil #2 \hfil}}


\newcommand{\columnimagestack}[2][1,.98]{%
  \@forlast\n@xtimg:=#2\do%
     {\makebox(0,0)[lb]{\mycolumnimage[#1][]{\n@xtimg}}}%
     {\mycolumnimage[#1][]{\n@xtimg}}%
}

%% so is scaleimage

\def\ScaleImgTwoOpt[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}

\def\ScaleImgOneOpt[#1,#2]{%
  \@ifnextchar[%]
    {\ScaleImgTwoOpt[#1,#2]}%
    {\ScaleImgTwoOpt[#1,#2][]}%
}

\def\scaleimage{%
  \@ifnextchar[%]
    {\ScaleImgOneOpt}%
    {\ScaleImgOneOpt[1,1]}%
}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% beamer extensions
\@ifclassloaded{beamer}{

%% Beamer controlled underbrace.  
%% \underbraceon<spec>[prefix]{maintext}{subtext}
%%   - prefix should probably live outside the \alt anyway
\newcommand<>{\underbraceon}[3][]{%
  \alt#4{%
    {#1{\underset{#3}{\underset{\text{\upbracefill}}{#2}}}}
  }{
    {#1{\underset{\phantom{#3}}{\underset{\phantom{\text{\upbracefill}}}{#2}}}}
  }%
}

} % end if beamer



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pgf extensions

\def\pgfp@nelparsearg[#1,#2]{%
  \def\pgfp@nelwidth{#1\panelwidth}%
  \def\pgfp@nelheight{#2\panelheight}}

\newenvironment{pgfpanel}[1][1,.995]
  {\pgfp@nelparsearg[#1]
   \begin{pgfpicture}{0cm}{0cm}{\pgfp@nelwidth}{\pgfp@nelheight}
      \pgftranslateto{\pgfpoint{0cm}{\pgfp@nelheight}}
      \pgfsetxvec{\pgfpoint{\pgfp@nelwidth}{0cm}}
      \pgfsetyvec{\pgfpoint{0cm}{-\pgfp@nelheight}}}
  {\end{pgfpicture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these use pgf to place a box at an arbitrary spot and (second form)
%% draw an arrow to the current position

\newcommand\placebox[4][left,baseline]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfputat{\pgfpoint{#2}{#3}}{\pgfbox[#1]{#4}}
  \end{pgfpicture}%
}

\newcommand\arrowbox[4][{0cm}{0cm}]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfnodebox{text}[virtual]{\pgfpoint{#2}{#3}}{#4}{2pt}{2pt}
    \pgfnodecircle{origin}[virtual]{\pgfpoint#1}{0pt}
    \pgfsetlinewidth{.5mm}
    \pgfsetendarrow{\pgfarrowsingle}
    \pgfnodeconnline{text}{origin}
  \end{pgfpicture}
}




% \def\alignmiddle#1{%
%   \setbox0=\hbox{#1}%
%   \dimen0=\dp0%
%   \advance\dimen0 by -\ht0%
%   \divide\dimen0 by 2%
%   \raise\dimen0\box0%
% }


\makeatother


==> m.symbols.tex <==
\RequirePackage{ifthen}

% use | for math mode
%\catcode`\|=3

% use textmode for a short minus sign
\newcommand{\tminus}{\text{\textendash}}

% vector
\newcommand{\vx}{\vec x}

% symbols for probability distributions
\newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
\newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
\newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}
% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\lr]{x} -> \mathbb{E}_a \lr[ x \lr]
\makeatletter
\def\expect{\@ifnextchar[{\expect@}{\expect@@[][\lr]}}
\def\expect@[#1]{\@ifnextchar[{\expect@@[#1]}{\expect@@[#1][\lr]}}
\def\expect@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{E}\newlr#2[{#3}#2]}%
             {\mathbb{E}_{#1}\newlr#2[{#3}#2]}}
\def\var{\@ifnextchar[{\var@}{\var@@[][\lr]}}
\def\var@[#1]{\@ifnextchar[{\var@@[#1]}{\var@@[#1][\lr]}}
\def\var@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{V}\newlr#2[{#3}#2]}%
             {\mathbb{V}_{#1}\newlr#2[{#3}#2]}}
\makeatother
\newcommand{\angles}[2][\lr]{{\newlr #1\langle{#2}#1\rangle}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathcal{E}}{=}}
% likelihoods
\newcommand{\like}[2]{\ensuremath{{\cal L}_{#1}\left({#2}\right)}}
\newcommand{\loglike}[2]{\ensuremath{\ell_{#1}\left({#2}\right)}}
\newcommand{\eff}{\mathcal{F}}
% info theoretic
\newcommand{\entropy}[2][\lr]{\ensuremath{\textbf{\textsf{H}}%
                             {\newlr #1[{#2}#1]}}}
\def\mutualinfo[#1;#2]{\ensuremath{\textbf{\textsf{I}}[{#1};{#2}]}}
\newcommand{\KL}[3][\lr]{\ensuremath{\textbf{\textsf{KL}}%
                             {\newlr #1[{#2}\lrmid #1\|{#3}#1]}}}
\newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
\newcommand{\normal}[3][\lr]{\ensuremath{\newlr\mathcal{N}#1(#2,#3#1)}}

% fractions
\newcommand{\half}{\ensuremath{{1\over2}}}
\newcommand{\overN}{\ensuremath{{1\over N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}

% whitened quantities
\newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\setV}{\ensuremath{{\cal V}}}
\newcommand{\setX}{\ensuremath{{\cal X}}}
\newcommand{\setY}{\ensuremath{{\cal Y}}}
\newcommand{\setZ}{\ensuremath{{\cal Z}}}
\newcommand{\size}[1]{\ensuremath{\left\vert{#1}\right\vert}}

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
\renewcommand{\vec}[1]{\ensuremath{\mathchoice%
{\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
{\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
\newcommand{\norm}[2][\lr]{\ensuremath{\newlr#1\|#2#1\|}}
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\renewcommand{\det}[2][\lr]{\ensuremath{\newlr#1\vert{#2}#1\vert}}
\newcommand{\trace}[2][\lr]{\ensuremath{\newlr\mathsf{Tr}#1[{#2}#1]}}
\newcommand{\diag}[2][\lr]{\ensuremath{\newlr\mathbox{\textsf{diag}}#1[{#2}#1]}}


% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\newcommand{\intdx}[1][dx]{\int\!\!#1\,}

\newcounter{multintctr}
\newcommand{\mltint}[1][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \int}

\newcommand{\mltintdx}[2][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \intdx[#2]}

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}


% accents

% adapted from symbols-a4.pdf; optional args permit shortening at left
% and right ends
\makeatletter
\def\widebar{\@ifnextchar[{\widebar@}{\widebar@@[3][0]}}
\def\widebar@[#1]{\@ifnextchar[{\widebar@@[#1]}{\widebar@@[#1][0]}}
\def\widebar@@[#1][#2]#3{{}\mkern#1mu\mkern#2mu\overline{\mkern-#1mu#3\mkern-#2mu}}
\makeatother    
        

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}


\newboolean{inlr}
\newboolean{midlr}
\setboolean{inlr}{false}
\newcommand\newlr{\setboolean{inlr}{false}}

\newcommand\lr[1]{%
  \ifthenelse{\boolean{inlr}}%
    {\ifthenelse{\boolean{midlr}}%
      {\middle#1\setboolean{inlr}{true}}
      {\right#1}}%
    {\left#1\setboolean{inlr}{true}}}%
\newcommand\lrmid{%
  \ifthenelse{\boolean{inlr}}%
    {\setboolean{midlr}{true}}
    {}}%


